Electronic Structure Evolution during the Growth of Graphene Nanoribbons on Au(110)

Surface-assisted polymerization of molecular monomers into extended chains can be used as the seed of graphene nanoribbon (GNR) formation, resulting from a subsequent cyclo-dehydrogenation process. By means of valence-band photoemission and ab-initio density-functional theory (DFT) calculations, we investigate the evolution of molecular states from monomer 10,10'-dibromo-9,9'bianthracene (DBBA) precursors to polyanthryl polymers, and eventually to GNRs, as driven by the Au(110) surface. The molecular orbitals and the energy level alignment at the metal-organic interface are studied in depth for the DBBA precursors deposited at room temperature. On this basis, we can identify a spectral fingerprint of C-Au interaction in both DBBA single-layer and polymerized chains obtained upon heating. Furthermore, DFT calculations help us evidencing that GNRs interact more strongly than DBBA and polyanthryl with the Au(110) substrate, as a result of their flatter conformation.

==> figures/a <==
Figure01}
UPS_DOSv6} 
energy_level_diagram}
figura3_1}
PA_BA_dos}&
poly_structure}\vspace{12pt}
AuP_2x1_bands}\hspace{0.03\textwidth}
AuP_2x1_rot_bands2}\hspace{0.03\textwidth}
BA_bands}\hspace{0.03\textwidth}
gnr_dos}&
gnr_structure}\vspace{12pt}
AuR_4x1_bands}\hspace{0.03\textwidth}
AuR_2x1_rot_bands2}\hspace{0.03\textwidth}
AuR_2x1_bands2}\hspace{0.03\textwidth}
TOC.png}

